AdBooster: Personalized Ad Creative Generation using Stable Diffusion Outpainting

In digital advertising, the selection of the optimal item (recommendation) and its best creative presentation (creative optimization) have traditionally been considered separate disciplines. However, both contribute significantly to user satisfaction, underpinning our assumption that it relies on both an item's relevance and its presentation, particularly in the case of visual creatives. In response, we introduce the task of {\itshape Generative Creative Optimization (GCO)}, which proposes the use of generative models for creative generation that incorporate user interests, and {\itshape AdBooster}, a model for personalized ad creatives based on the Stable Diffusion outpainting architecture. This model uniquely incorporates user interests both during fine-tuning and at generation time. To further improve AdBooster's performance, we also introduce an automated data augmentation pipeline. Through our experiments on simulated data, we validate AdBooster's effectiveness in generating more relevant creatives than default product images, showing its potential of enhancing user engagement.

==> misc.tex <==
\begin{abstract}
Digital advertising requires personalization, yet existing methods often overlook the creative content's personalization. To address this, we introduce the task of \emph{Generative Creative Optimization (GCO)}, that is able to leverage user interest signals for tailored creative generation. Furthermore, we propose 
\emph{AdBooster}, a model for personalized ad creatives, founded on the StableDiffusion outpainting architecture, and uniquely incorporating individual user interest distribution during fine-tuning. We also introduce an automated data augmentation pipeline to boost AdBooster's performance. Our extensive experiments validate AdBooster's superiority in generating more relevant creatives compared to default product images, leading to enhanced user engagement. Thus, with GCO, automated data augmentation, and StableDiffusion architecture, AdBooster holds the potential to revolutionize ad creative generation.
\end{abstract}



\subsection{Evolutionary Search}

\paragraph{Notation:}
\begin{itemize}
    \item $\pi_\theta(a|s)$ is the deterministic policy that determines what action to take in state s (stochastic policies are supported by supplementing the input parameters in $\theta$ with a random seed $\epsilon$)
    \item $\tau(\theta)$ is a trajectory fully specified by the policy parameters $\theta$ and representing the sequences of actions and states, denoted as $\mathbf{a}$ and $\mathbf{s}$
    \item $R(\tau(\theta))$ is the reward from a particular policy trajectory following the policy parametrised by $\theta$
    \item $J(\theta)$ is the expected reward over $\theta$: $ J(\theta)
    = \E_{\theta} [ R(\tau(\theta))]$
\end{itemize}


\paragraph{Reco-RL as A/B test automation}
If we are interested in improving our Reco policy:
\begin{itemize}
    \item strictly online
    \item fully automatic
\end{itemize}
then an Evolutionary Strategy approach is perfectly suited:


\paragraph{ES-based formulation:}
\begin{itemize}
    \item $p(\theta|\psi)$ is the conditional distribution of the potential policies fully defined by their parameters $\theta$ and with its own parameters $\psi$ (usually representing the mean and variance of a Gaussian distribution).
    \item Goal: to maximize the expected value of the solutions in the population: $\E_{\theta \sim p(\theta|\psi)} J(\theta)$
\end{itemize}


\paragraph{ES Gradient Ascent:}
\begin{equation}
\begin{split}
    \nabla_\psi J_{ES}(\psi) 
    = \E_{\theta \sim p(\theta|\psi)} [ R(\tau(\theta))\nabla_\psi \log p(\theta|\psi) ] = \\
    \approx \frac{1}{N} \sum_{n=1}^N R(\tau(\theta_n))\nabla_\psi \log p(\theta_n|\psi)
\end{split}
\end{equation}


\paragraph{ES Gradient Ascent Vanilla:}

$\nabla_\psi \log p(\theta_n|\psi)$ can be computed as:
\begin{itemize}
    \item $\nabla_{\mu_n} \log p(\theta|\psi) = \frac{\theta_n - \mu_n}{\sigma^2_n} = \frac{\epsilon_n\sigma_n}{\sigma^2_n}$ , $\nabla_{\sigma_n} \log p(\theta|\psi) = \frac{(\theta_n - \mu_n)^2-\sigma^2_n}{\sigma^3_n}$
\end{itemize}

We have then that:
\begin{equation}
\begin{split}
    \nabla_\psi J_{ES}(\psi) 
    \approx \frac{1}{N} \sum_{n=1}^N R(\tau(\theta_n))\nabla_\psi \log p(\theta_n|\psi) = \\
    = \frac{1}{N\sigma_n} \sum_{n=1}^N R(\tau(\mu_n + \sigma_n\epsilon_n))\epsilon_n 
\end{split}
\end{equation}

\paragraph{ES Gradient Ascent with Antithetic Sampling:}
where $\nabla_\psi J_{ES}(\psi)$ can be computed via finite differences (as a central difference):

\begin{equation}
\begin{split}
    \nabla_\psi J_{ES}(\psi) 
    \approx \frac{1}{N\sigma_n} \sum_{n=1}^N \frac{R(\tau(\mu_n + \sigma_n\epsilon_n)) - R(\tau(\mu_n - \sigma_n\epsilon_n))}{2}\epsilon_n
\end{split}
\end{equation}
This has a lot less variance, as shown in \href{http://www.argmin.net/2017/04/03/evolution/}{Ben Recht's post on ES}.


%For more details, see \cite{salimans2017evolution} and \cite{sehnke2010parameter}.


\RestyleAlgo{ruled}
\begin{algorithm}[hbt!]
\caption{Reco-ES Algorithm}\label{alg:ES}


1. \textbf{Hyperparameters:} step-size $\alpha$, standard deviation of the noise $\sigma$, number of directions $N$, max nb. iterations $jmax$\\
2. \textbf{Initialize:} $\theta_0 = Prod, j = 0$ \\
3. Split users in 2N random sub-populations ( optionally stratified by \text{NbDisplays})\\
4. \While{j \leq jmax}{
5. Sample jitter noise \epsilon_1, \epsilon_2 ... \epsilon_N; \\
6.  Run 2N randomized policies of the form $\pi_{\theta_j+\sigma\epsilon_i}$, $\pi_{\theta_j-\sigma\epsilon_i}$ on the 2N sub-populations\\
7. Collect pairs of rewards $r({\theta_j+\sigma\epsilon_i}), r({\theta_j-\sigma\epsilon_i})$ \\
8.  Update $theta$: $\theta_{j+1} = \theta_j + \frac{\alpha}{N}\sum_{n=1}^N [r({\theta_j+\sigma\epsilon_i}) - r({\theta_j-\sigma\epsilon_i})]\epsilon_i$ \\
9   .  j = j+1\\
}
\end{algorithm}



For a more advanced algorithm, we can check Ben Recht's paper on \emph{\href{https://arxiv.org/pdf/1803.07055.pdf}{Simple random search provides a competitive approach
to reinforcement learning}} \cite{mania2018simple}.

\paragraph{Policy Gradient (PG)}

\paragraph{REINFORCE Algorithm}


\paragraph{REINFORCE Gradient Ascent}

\begin{equation}
\begin{split}
    \nabla_\theta J_{PG}(\theta) = \E_{\tau \sim \pi_\theta} [ \sum_{t=0}^T R(\tau_t) \nabla_\theta \log \pi_\theta(a_{t}|s_{t})] = \\
     = \frac{1}{N} \sum_{n=1}^N  \sum_{t=0}^T R(\tau_{nt}) \nabla_\theta \log \pi_\theta(a_{nt}|s_{nt})
\end{split}
\end{equation}

For a good critique of PG and REINFORCE see again, Ben Recht's post on the \href{http://www.argmin.net/2018/02/20/reinforce/}{matter}.


\newpage
\paragraph{ES vs. PG}


\begin{itemize}
\item  The advantage of the ES approach is that
the actions are deterministic, and an entire history can therefore be generated from a single parameter sample. This reduction in samples-per-history is what reduces the variance in the gradient estimate: in PG, the variance of the gradient is proportional to a sum of T uncorrelated terms, so that the variance of the policy gradient estimator will grow nearly linearly with T. The corresponding term for ES is independent of T.


\item As an added benefit the parameter gradient is estimated by direct parameter perturbations, without having to back-propagate any derivatives, which allows the use of non-differentiable policies.
\end{itemize}




\subsection{Clicky Reco vs. Causal Reco}


\begin{equation}
    
    
    \Delta_{ij} = CTR_i(j) \times CR_i(j) 
    \times \frac{CR_i(j) - CRNR_i(j)}{CR_i{j}}
    
    
    
\end{equation}


\paragraph{Ways to fine-tune $G_\theta$:}

\begin{itemize}
    \item Fine-tuning the generator $G_{\theta_}(i,t,\epsilon)$ by: 
    \begin{itemize}
        \item   Learning a projection matrix from the original conditioning CLIP-space to a new space that is monotonically related to $R(.)$ (a la WARHOL).

    \item Learning a projection matrix from the original pre-decoder latent space to a new space that is monotonically related to $R(.)$:
    \begin{equation}
    \theta_1^* = \argmax_{\theta_1} \sum_s R(G_{\theta_1}(t_{\theta_2}(x,s),i(x),\epsilon),s)
    \end{equation}

    \end{itemize}
    
    \item Fine-tuning the text prompt $t_{\theta_2}(x,s)$  model by: 
    \begin{itemize}
        \item  overwriting the embedding of the dedicated token for the product $x$ (see DREAMBOOTH)
        \item learning a better token transition model that increases the quality of the generation and the resulting reward
    \end{itemize}

    \begin{equation}
    \theta_2^* = \argmax_{\theta_2} \sum_s R(G_{\theta_1}(t_{\theta_2}(x,s),i(x),\epsilon),s)
    \end{equation}
    
\end{itemize}


\paragraph{Ways to condition $G_\theta$:}
\begin{itemize}
    \item Add a textual description of the context to the input prompt (or add a reserved keyword)
    
    
    
\end{itemize}

The resulting prompt will be of the type: \emph{ad of [product category] [x] for [demographic group s], [additional text determined by the text prompt generator]}. 


\subsection{Online RL reward optimization}
\begin{itemize}
    \item \href{https://arxiv.org/pdf/1703.03864.pdf}{OpenAI ES paper}\cite{salimans2017evolution}
    \item \href{https://mediatum.ub.tum.de/doc/1287490/1287490.pdf}{Parameter-exploring Policy Gradients paper}\cite{sehnke2010parameter}
    \item \href{https://openai.com/blog/evolution-strategies/}{Lilian's Weng blogpost on ES for RL}
    \item \href{https://openai.com/blog/evolution-strategies/}{OpenAI Blog post on ES}
    \item \href{https://www.inference.vc/evolutionary-strategies-embarrassingly-parallelizable-optimization/}{Ferenc Huznar's blogpost on ES}
    \item \href{https://colab.research.google.com/drive/1SY38Evy4U9HfUDkofPZ2pLQzEnwvYC81?usp=sharing}{Simple Colab implementation}
\end{itemize}


\subsection{Image Reward models}
\begin{itemize}
    \item \href{https://towardsdatascience.com/perceptual-losses-for-image-restoration-dd3c9de4113}{Perceptual Loss} 
    \item \href{https://github.com/crowsonkb/simulacra-aesthetic-models}{Aesthetic Model}
\end{itemize}


\paragraph{Ways to fine-tune $G_\theta$:}


\todo{ToDo: List the existing ways of fine-tuning the stable diffusion model (classic \& outpainting)}


\paragraph{Ways to condition $G_\theta$:}
\begin{enumerate}
  
    \item By adding a textual description of the context to the input prompt (or add a reserved keyword) The resulting prompt will be of the type: \emph{ad of [product category] [x] for [demographic group s], [additional text determined by the text prompt generator]}. 

    \item ...
    
    
\end{enumerate}

\todo{ToDo: List possible ways of conditioning the stable diffusion model (classic \& outpainting)}


\subsection{The optimization}

\subsubsection{Model-based methods}

Model-based optimization assumes that we have a prebuilt model for the reward $R(.,.)$.
Once the model is built we can directly optimize $\theta$ using the equations in the previous subsection.
In the case where a reward-model is hard to build we can directly learn the $\theta$ online using one of the following methods.


\subsubsection{On-policy RL methods}



\subsection{ The generative model $G_\theta$}

We assume that the image generative model $G_\theta(x,s) = G_{\theta}(i_{\theta_1}(x), t_{\theta_2}(x,s),\epsilon)$ 
is a CLIP-conditioned image diffusion model such as StableDiffusion, that takes as input: 
\begin{itemize}
    \item a CLIP-encoded image seed $i_{\theta_1}(x)$ 
    \item a CLIP-encoded text prompt $t_{\theta_2}(x,s)$
    \item a noise vector $\epsilon$.
\end{itemize}

